Self-Supervised Anomaly Detection by Self-Distillation and Negative Sampling

Detecting whether examples belong to a given in-distribution or are Out-Of-Distribution (OOD) requires identifying features specific to the in-distribution. In the absence of labels, these features can be learned by self-supervised techniques under the generic assumption that the most abstract features are those which are statistically most over-represented in comparison to other distributions from the same domain. In this work, we show that self-distillation of the in-distribution training set together with contrasting against negative examples derived from shifting transformation of auxiliary data strongly improves OOD detection. We find that this improvement depends on how the negative samples are generated. In particular, we observe that by leveraging negative samples, which keep the statistics of low-level features while changing the high-level semantics, higher average detection performance is obtained. Furthermore, good negative sampling strategies can be identified from the sensitivity of the OOD detection score. The efficiency of our approach is demonstrated across a diverse range of OOD detection problems, setting new benchmarks for unsupervised OOD detection in the visual domain.

==> fig/auroc_10nn.tex <==
\begin{figure}[t]
\begin{center}

\includegraphics[width=.97\columnwidth]{fig/AUROC_10NN_cifar10_cifar100.pdf}
\end{center}
\caption{$10$-NN for CIFAR$10$ training dataset and  anomaly detection AUROC scores of near OOD CIFAR$100$ samples for different $\mathcal{D}_{neg}$: Shuffle, Perm-$16$, Perm-$4$, RotPerm-$4$, DINO, Aux 1, Rot Aux 1, Aux 2, Combined, Rot. In-Dist respectively. In near OOD regime, AUROC score is  correlated with KNN performance. In-distribution negative samples increse both KNN accuracy and anomaly detection AUROC score for near OOD samples.}

\label{fig:auroc_10nn}
\end{figure}

==> sec/X_instructions.tex <==
% --- repeat the title (AT: haven't found a more elegant way to do this...)
\twocolumn[
\centering
\Large
\textbf{\LaTeX\ Author Guidelines for \confName~Proceedings (2022)}
\vspace{1.0em}
] %< twocolumn
\appendix

\setcounter{section}{0}
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of cvpr.sty to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the CVPR70 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.


% Update the cvpr.cls to do the following automatically.
% For this citation style, keep multiple citations in numerical (not
% chronological) order, so prefer \cite{Alpher03,Alpher02,Authors14} to
% \cite{Alpher02,Alpher03,Authors14}.


\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}

%------------------------------------------------------------------------
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

%------------------------------------------------------------------------
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/comments.tex <==
%%%% SECTION 4.3
% under construction - we can still remove it
% Our results highlight that rotation helps making negative samples dissimilar to the in-distribution in terms of high-level semantic, which forces the model to have a more compact representation for in-distribution features by contrasting against the negative examples
% perm related
% standard and all patch and pixel-wise permutations of the ImageNet auxiliary dataset. 
% Moreover, we found that  ImageNet images as negatives result in better performance than applying jigsaw with 4 and 16 patch splits. we highlight that Perm-$16$ almost always improves the OOD performance compared to jigsaw with $4$ patches and on par with the random shuffling of image pixels.
%As depicted in table \ref{tab:contrast_dataset_cif10}, the performance degrades when we use standard ImageNet compared to rotated one. On the other hand,  Interestingly we found that jigsaw with $16$ patches split almost always improves the OOD performance compared to jigsaw with $4$ patches and on par with the random shuffling of image pixels. On the contrary, rotated CIFAR$10$ examples outperform standard and all patch and pixel-wise permutations of the ImageNet auxiliary dataset. However, provide inferior results compared to rotated ImageNet excluding CIFAR$100$ OOD data.  
% The reason can be explained by the fact that we are not using any label information 
% where there is a high chance to have negative samples semantically similar to in-distribution data like using ImageNet without any rotation. 
% One issue with nonrot ImageNet as auxiliary dataset is that negative samples might have significant similarity with in-distribution data which can force the model to consider in-distribution test samples as negative during the evaluation phase which results in performance deterioration. 
% We further study this by applying jigsaw transformation with 4 patches. With this transformations each auxiliary sample is divided into 4 patches and then is permuted. This augmentation still contains image semantics to some extend and can share considerable similarities with CIFAR$10$
% results in worse average performance compare to when we use jigsaw with 16 patches or even when we completely destroy the semantic by random pixel shuffling of ImageNet samples. We saw that rotating the jigsaw with 4 patches improves the average performance which again confirms the above argument about effect of negative samples with high similarity to in-distribution data. 
% We could outperform all other methods where we train on CIFAR$10$ when we use combination of rotated in-distribution samples and rotated ImageNet as negative examples. 
% % compare three different negative  in-dist , combine , auxiliary for near ood and far ood 
% In addition, we could exceed other self-supervised methods for the case of CIFAR$100$ as in-distribution where we use auxiliary rotated ImageNet samples as negative compared to where we include rotated in-distribution data as negative.
% In Table \ref{tab:contrast_dataset_cif10}, we conduct experiments on different variations of auxiliary dataset from which we drive the negative examples and we compare them with the vanilla DINO where we don't have any negative examples. As it is clear from the table combination of rotated ImageNet images and rotated in-distribution samples achieves the highest AUROC score for the near-OOD detection task of CIFAR$10$ against CIFAR$100$ and also competing average AUROC. 

%\input{tab/imagenet30_sota}




% discussion

% trade-off
% Even though the proposed method works with either or a combination of them, we report this trade-off as a promising research direction for future work. Nonetheless, the combination poses extra computational complexity that one has to consider.
%does 
% Thus,\@ given a prior knowledge of which transformation forms good in-distribution negatives can yield superior near-OOD scores than by leveraging auxiliary data.\@ 
% far-ood
% We argue that rotation of a given CIFAR$10$ sample can form a negative example which resemble CIFAR$100$ samples more compared to rotation of an auxiliary ImageNet sample. 
% This can slightly enforce the model to capture more of higher level semantics. But with use of rotated auxiliary Imagenet samples, as we are not using any label information, there exists smaller chance of contrasting a sample with negative one of the same category although, rotated ImageNet samples as negative can resemble many OOD dataset due to broad distribution it has. Thus, make it a better choice for far OOD data. 
% Having CIFAR10 as in-distribution training data, in Table \ref{tab:10-NN_table} we show that there is a direct correlation between the performance on OOD detection of and KNN accuracy. This is in line with results in \cite{robinson2021contrastive, hard_negative_mixing} where they show that utilising hard negative samples can improve the representation learned by contrastive methods. 
% \input{tab/10-NN}
% \input{fig/auroc_10nn}
% \subsection{Discussion on Latent Space (Clustering) Improvement}
% Figure \ref{tsneplot} shows a two-dimensional t-SNE visualization of feature space when model trained on CIFAR$10$. (need to complete)
% We can observe that representations obtained by minimizing our proposed loss are more befitted for OOD detection as it leads to a more compact representation of in-distribution data.
%\input{tab/table2_comparison_AUROC_OOD} % overlapping-patches
%\input{tab/table3_comparison_KNN_patches} % v2, overlapping-patches
%\input{tab/table5_AUROC_without_label_supervision} % overlapping-patches
%\input{tab/table6_v2_temp_imagenet} % V2 Imagenet30
%\input{tab/table7_D_in_train_Imagenet}
%\input{tab/table8_v2_temp_cifar100} % V2 Cifar100
%\input{tab/table9_D_in_train_Cifar100}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sec 3






%In addition, we conduct extensive experiments on different transformations which could be 


% The reason to use rotation is that within the regime of objective centric images we can remove semantic similarities with in-distribution data otherwise the model learns to reject in-distribution test data during the evaluation by considering them as negative. 
% . later we explain the auxiliary objective in more details. 

% Shifting transformations can be applied on both in-distribtuion and on auxiliary data samples. Forming negative examples from in-distribtuion data can result in so-called hard negatives as they share more low-level statistics with positive samples and can force the model to capture higher level of semantics in order to be able to distinguish between positive and negative samples which can result in a more robust representation\cite{robinson2021contrastive}. This is challenging task as it needs more dataset specific knowledge as  





% In the case of applying on in-distribution data we need specific dataset prior knowledge to make sure that transformation is changing the semantic.  

% In specific we introduce negative examples to model such that 
% To form the negative samples we either apply rotation as a shifting transformation on in-distribution data or on an auxiliary dataset like ImageNet. 

% This can result in a more conservative decision boundary of in-distribution data \cite{HendrycksMD19}. The harder the negative sample distribution is the more conservative the model decision boundary for in-dist data will be\cite{robinson2021contrastive}. One of the main challenges with creating hard negatives is that negative samples should not be completely similar to in-distribution data otherwise the model learns to reject in-distribution test data during the evaluation phase by considering them as negative samples. Subject to this we can argue that by having more prior knowledge about the dataset we can design more effective hard and correct negatives.
% For instance, it is shown \cite{mohseni2021shifting} that rotation can be considered as an effective shifting transformation for CIFAR10. This also can be understood intuitively as there is not any category in CIFAR10 that preserves the semantic under rotation transformation. On the other hand, rotation is not helpful when training on CIFAR100 where we have categories like keyboard, orange. These categories have examples that remain the same under rotation. [some figure from cifar100]


 




% \subsection{Negative sampling}
% The proposed method aims to enhance DINO's learned representation by adding negative samples. The natural question would be how to construct the appropriate views to contrast on. In this direction, we investigate if providing auxiliary dataset (aux-dist) can be leveraged. In our best setup, we apply the same set of transformations $T$ plus a random rotation $r \sim R = \{ 90^{\circ}, 180^{\circ}, 270^{\circ} \}$. The reason is two-fold: a) to alter the semantics so no semantics are shared between in-distribution and aux-dist, b) to ...

% We also experimented with .... 

% In more detail, $N$ local and 1 global negative views are passed to the student network. 



% \subsubsection{Proposed auxiliary loss}
% After creating the negative samples,



% In this direction, we use 
% (explain imagenet to include less dataset-specific knowledge and explain including more dataset-specific knowledge like rotation for cifar10 and probably translation for cifar100
%  )

% ImageNet (as a universal set of images). There is a high chance that there exist class category overlaps between ImageNet and most of the existing image datasets which can force the model to reject test samples of in-dist data. To overcome this issue we apply randomly selected rotation $r$ where $r \sim R = \{ 90^{\circ}, 180^{\circ}, 270^{\circ} \}$.



==> tab/10-NN.tex <==
\begin{table}[ht]
%\begin{wraptable}{r}{0.5\linewidth}
%\LARGE
\caption{$10$-NN for CIFAR$10$ training dataset vs  anomaly detection AUROC scores of near OOD CIFAR$100$ samples for different $\mathcal{D}_{neg}$. In near OOD regime, AUROC score is  correlated with KNN performance. Harder negative samples increse both KNN accuracy and anomaly detection AUROC score for near OOD samples.}
\vspace{-0.5cm}
\label{tab:10-NN_table}
\setlength{\tabcolsep}{2pt}
\begin{center}
\begin{tabular}{lcc}
%{0.75\linewidth}{c*{2}{Y}}
\hline
%&\multicolumn{2}{c}{$10$-NN Classifier}
%\\
% \cline{2-3}
\multicolumn{1}{c}{$\mathcal{D}_{neg}$} & $10$-NN & AUROC
\\
\hline
\multirow{3}{*}{}
Pixel-shuffled ImageNet & $90.89$ & $87.67$ \\
Jigsaw-$16$ &  $91.09$ & $88.32$ \\
Jigsaw-$4$ & $91.93$ & $89.57$ \\
Jig-$4$-Rot & $92.31$ & $89.29$ \\
Vanilla DINO& $93.24$ & $90.29$ \\
ImageNet & $93.36$ & $90.46$ \\
Rotated ImageNet& $94.35$ & $92.51$\\
Debiased TinyImageNet& $94.88$ & $93.77$ \\
Rotated ImageNet+Rotated In-Dist & $95.88$ & $94.20$ \\
Rotated In-Dist &  $95.99$ & $93.96$ \\

\hline
\end{tabular}
%\end{adjustbox}
%} % end resize box
\end{center}
%\end{wraptable}
\end{table}

==> tab/cifar100_Ablation_table.tex <==
\begin{table*}[t]
\label{tab:contrast_dataset_cif100}
\caption{AUROC scores for OOD Detection with CIFAR$100$ as {$\mathcal{D}^{in}_{train}$} and different $\mathcal{D}_{neg}$. ImgN denotes ImageNet samples.} 
\setlength{\tabcolsep}{2pt}
\begin{center}
\begin{tabularx}{\linewidth}{c*{11}{Y}}
\hline

\multicolumn{2}{c|}{Negative Sampling:} &  \multicolumn{1}{Y|}{None} & \multicolumn{8}{c|}{Auxiliary} & \multicolumn{1}{Y}{In-Dist} \\
\hline
\parbox[t]{1.0cm}{\centering \medskip \smallskip $\mathcal{D}_{train}^{in}$}  &
\parbox[t]{1.85cm}{\centering \medskip \smallskip $\mathcal{D}_{test}^{out}$ } &  DINO  $\lambda=0$ & ImgN & Rot. ImgN & Rot.$360$ ImgN & DTI & Perm-$16$ ImgN & Perm-$4$ ImgN & \parbox[t]{1.0cm}{\centering Rot.\\DTI} & Pix. Perm. & Rot. In-Dist. \\

\hline

\multirow{11}{*}{} 
\multirow{8}{*}{\rotatebox{90}{CIFAR$100$}}

&
  \multicolumn{1}{c}{CIFAR$10$} &
                   $69.69$ & $69.29$ & $69.96$ & $70.47$ & $70.51$ & $70.37$ & $69.61$ & $69.08$ & $\mathbf{70.64}$ & $67.63$\\ % & $67.63$ \\
                   
& \multicolumn{1}{c}{SVHN} &  
                   $89.28$ & $90.30$ & $96.00$ & $95.22$ & $96.61$ & $96.39$ & $95.33$ & $97.47$ & $96.91$ & $\mathbf{97.95}$\\

& \multicolumn{1}{c}{ImageNet$30$} & 
                   $69.78$ & $71.80$ & $\mathbf{84.82}$ & $79.20$ & $76.36$ & $73.38$ & $77.00$ & $76.35$ & $74.65$ & $75.36$ \\

& \multicolumn{1}{c}{TinyImageNet} & 
                   $73.94$ & $80.25$ & $81.41$ & $80.84$ & $77.92$ & $75.26$ & $\mathbf{81.93}$ & $80.20$ & $76.28$ & $79.75$  \\           
                   
& \multicolumn{1}{c}{LSUN} & 
                   $65.43$ & $72.38$ & $\mathbf{85.03}$ & $78.01$ & $78.11$ & $70.70$ & $76.61$ & $76.99$ & $72.80$ & $74.55$  \\          

& \multicolumn{1}{c}{STL$10$} & 
                    $70.18$ & $69.14$ & $\mathbf{79.96}$ & $76.10$ & $71.58$ &  $70.49$ & $73.73$ & $69.30$ & $72.58$ & $71.70$  \\

& \multicolumn{1}{c}{Places$365$} & 
                   $67.30$ & $70.44$ & $\mathbf{81.67}$ & $77.89$ & $77.99$ & $71.43$ & $75.92$ & $75.54$ & $73.30$ & $72.79$  \\

& \multicolumn{1}{c}{Texture} & 
                   $55.73$ & $67.83$ & $\mathbf{80.65}$ & $67.76$ & $64.52$ & $61.42$ & $69.89$ & $73.36$ & $64.01$ & $77.33$  \\

\hline
& \multicolumn{1}{c}{Average} & 	
                   $69.85$ & $73.16$ & $\mathbf{82.44}$ & $78.13$ & $76.85$ &
                   $73.43$ & $77.21$ & $77.09$ & $74.95$ & $76.57$ \\
            
\hline
\end{tabularx}
%\end{adjustbox}
%} % end resize box
\end{center}
\label{tab:contrast_dataset_cif100}
\end{table*}



%  & $97.17$ \\


%  & $75.36$ \\


% TinyImageNet & 
%                    & $79.75$ \\                   
% %\multirow{10}{*}{}& 
% LSUN & 
%                   & $74.55$ \\
% %\multirow{10}{*}{}& 
% STL$10$ & 
%                   & $71.70$ \\
% %\multirow{10}{*}{}& 
% Places$365$ & 
%                   $00.00$ & $70.44$ & $\mathbf{81.67}$ & $00.00$ & $77.55$ & $71.43$ & $75.92$ & $69.37$ & $73.30$ & $71.54$ & $72.79$ \\
% Texture & 
%                   $00.00$ & $67.83$ & $\mathbf{80.65}$ & $00.00$ & $65.35$ & $61.42$ & $69.89$ & $61.497$ & $64.01$ & $77.00$ & $77.33$ \\
% %\hline
% %Average & 	
% %                   $00.00$ & $73.16$ & $\mathbf{82.38}$ & $00.00$ & $76.73$ & %$73.43$ & $77.21$ & $72.03$ & $74.95$ & $75.07$ & $76.57$ \\

==> tab/cifar10_portion_ImgN.tex <==
\begin{table*}[t]
\caption{AUROC OOD Detection score (\%) and KNN accuracy for with CIFAR$10$ as $\mathcal{D}_{train}^{in}$ and Rot. Imagenet as $\mathcal{D}_{neg}$. $p$ indicates the percentage of the ImageNet samples (1.2M) used.} 
\label{tab:cif10_portion_ImgN}
\setlength{\tabcolsep}{2pt}
\begin{center}
\begin{tabularx}{\linewidth}{c*{10}{Y}}
\hline
\parbox[t]{1.0cm}{\centering \medskip \smallskip $\mathcal{D}_{train}^{in}$}  &
\parbox[t]{1.85cm}{\centering \medskip \smallskip $\mathcal{D}_{test}^{out}$ } & $p=1\%$ & $p=5\%$ & $p=10\%$ & $p=20\%$ & $p=40\%$ & $p=60\%$ & $p=80\%$\\

\hline

\multirow{11}{*}{} 
\multirow{9}{*}{\rotatebox{90}{CIFAR$10$}}

& \multicolumn{1}{c}{CIFAR$100$} &
                   $92.39$ & $92.56$ & $\mathbf{93.03}$ & $92.63$ &
                   $92.67$ & $92.30$ & $92.86$ \\
                  
& \multicolumn{1}{c}{SVHN} &  
                   $99.59$ & $\mathbf{99.79}$ & $99.74$ & $99.68$ &
                   $99.67$ & $99.63$ & $99.77$  \\

& \multicolumn{1}{c}{ImageNet$30$} & 
                   $93.75$ & $94.35$ & $93.24$ & $93.50$ &
                   $\mathbf{94.37}$ & $94.19$ & $94.36$  \\

& \multicolumn{1}{c}{TinyImageNet} & 
                   $95.59$ & $\mathbf{96.36}$ & $95.92$ & $96.24$ &
                   $96.28$ & $95.99$ & $96.28$  \\                   

& \multicolumn{1}{c}{LSUN} & 
                   $98.19$ & $97.91$ & $97.67$ & $97.32$ &
                   $\mathbf{98.33}$ & $98.22$ & $98.26$  \\                   

& \multicolumn{1}{c}{STL$10$} & 
                   $78.11$ & $77.49$ & $75.80$ & $76.59$ &
                   $\mathbf{78.22}$ & $77.83$ & $77.64$  \\

& \multicolumn{1}{c}{Places$365$} & 
                   $96.98$ & $96.82$ & $96.36$ & $96.26$ &
                   $97.05$ & $97.08$ & $\mathbf{97.18}$  \\

& \multicolumn{1}{c}{Texture} & 
                   $98.68$ & $\mathbf{99.31}$ & $98.76$ & $98.75$ &
                   $98.66$ & $98.98$ & $99.17$ \\

\hline
& \multicolumn{1}{c}{Average} & 	
                   $94.47$ & $94.60$ & $94.08$ & $94.11$ &
                   $94.69$ & $94.57$ & $\mathbf{94.73}$ \\
\hline
\hline
& \multicolumn{1}{c}{KNN} & 
                    $94.16$ &
                    $94.25$ &
                    $94.54$ &
                    $94.46$ &
                    $94.42$ &
                    $94.40$ &
                    $\mathbf{94.55}$ \\
            
\hline
\end{tabularx}
%\end{adjustbox}
%} % end resize box
\end{center}
\end{table*}

==> tab/imagenet30_sota.tex <==
\begin{table}[ht]
\caption{OOD detection performance (AUROC $\%$) without label supervision,\@ $\mathcal{D}_{train}^{in}$: ImageNet$30$.\@ Rot.Aux refers to rotated ImageNet, Rot.In-Dist to rotated In-Distribution and Rot.(Aux+In.Dist) to a combined version of the former and the latter.}
\label{ImageNet30_sota}
\begin{center}
\begin{tabularx}{\linewidth}{l c*{3}{Y}}
\hline
%&&&&\multicolumn{2}{c}{\textbf{Ours}} \\
%\cline{4-5}
{$\mathcal{D}_{test}^{out}$} & CSI & MTL & \parbox[t]{2cm}{Rot. Aux} & Combined \\%& \parbox[t]{2cm}{Rot.\\In-Dist} \\  
\hline
% ImageNet30 as in dist
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



Flowers & 
                  $\mathbf{94.70}$ & $94.19$ &
                  $90.63$ & $93.82$ \\
                  %& $90.59$ \\

CUB-$200$ & 
                  $90.50$ & $\mathbf{93.34}$ &
                  $83.93$ & $84.67$ \\ 
                  % &$79.81$\\                  

Dogs & 
                  $\mathbf{97.10}$ & $93.63$ &
                  $87.29$ & $82.82$ \\
                  % $80.18$ \\

Food-$101$ & 
                  $\mathbf{89.20}$ & $82.51$ &
                  $81.71$ & $83.73$ \\
                  %&$83.38$ \\
 
Pets & 
                  $85.20$ & $\mathbf{94.82}$ &
                  $91.58$ & $87.98$ \\
                  % &$85.98$ \\

Caltech-$256$ & 
                  $\mathbf{87.10}$ & $-$ &
                  $85.46$ & $80.95$ \\
                  %&$79.11$ \\

Places$365$ & 
                  $\mathbf{78.30}$ & $-$ &
                  $77.17$ & $70.45$ \\ 
                  %&$70.84$ \\

Texture & 
                  $-$ & $\mathbf{93.99}$ &
                  $95.87$ & $93.34$ \\  
                  %&$90.32$\\
%\hline
%Average & 
%                  $-$ & $-$ &
%                  $\mathbf{85.25}$ & $84.61$  &
%                  $82.53$ \\ % $88.87$ avg CSI, $\mathbf{92.08}$ avg MTL
\hline
\end{tabularx}
\end{center}
\end{table}

==> tab/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tab/old_cifar100_Ablation_table.tex <==
\begin{table*}[t]
%\LARGE
\caption{AUROC scores for OOD Detection with CIFAR$100$ as {$\mathcal{D}_{train}^{in}$} and different $\mathcal{D}_{neg}$. Here, Rotated (Rot.,R) denotes rotated ImageNet images, Debiased is the debiased TinyImageNet dataset, the number after Jigsaw refers to the respective patches, Pixel means that the pixels have been shuffled, In-Dist refers to negative In-Distribution examples and lastly, R.+In-Dist is a combination of the latter one and rotated images.}
\label{tab:contrast_dataset_cif100}
\setlength{\tabcolsep}{2pt}
\begin{center}
%\resizebox{\linewidth}{!}{
%\resizebox{17cm}{2cm}{ % resize table
%\begin{adjustbox}{width=1\textwidth}
%\renewcommand{\arraystretch}{0.3} %change the spacing between rows
\begin{tabularx}{\linewidth}{c*{10}{Y}}
\hline
\multicolumn{1}{c}{$\mathcal{D}_{train}^{in}$: Cifar$100$} &&\multicolumn{7}{c}{OOD Detection AUROC ($\%$)}
\\
\cline{2-10}
%\multicolumn{1}{c}{$\mathcal{D}_{train}^{in}$} & 
%\multicolumn{1}{c}{$\mathcal{D}_{test}^{out}$} & Vanilla & Normal & Rotated & Debiased & Jigsaw-$16$& Jigsaw-$4$ & Pixel & In-Dist & R.+In-Dist\\
\multicolumn{1}{c}{$\mathcal{D}_{test}^{out}$} & Vanilla & Normal & Rotated & Debiased & Jigsaw-$16$ & Jigsaw-$4$ & Jig-$4$-Rot & Pixel & In-Dist & R.+In-Dist\\
\hline
% cifar10 as in dist
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\multirow{10}{*}{} 
CIFAR$10$ &
                   $00.00$ & $69.29$ & $00.00$ & $70.55$ &
                   $70.44$ & $69.61$ & $70.64$ & $00.00$ &
                   $00.00$ \\
%\multirow{10}{*}{}& 
SVHN &  
                   $00.00$ & $90.30$ & $00.00$ & $96.05$ &
                   $95.85$ & $95.33$ & $96.91$ & $00.00$ &
                   $00.00$ \\
%\multirow{10}{*}{}& 
ImageNet$30$ & 
                   $00.00$ & $93.28$ & $00.00$ & $85.24$ &
                   $94.99$ & $90.41$ & $92.09$ & $00.00$ &
                   $00.00$ \\
%\multirow{10}{*}{}& 
TinyImageNet & 
                   $00.00$ & $74.27$ & $00.00$ & $78.93$ &
                   $80.18$ & $75.18$ & $70.40$ & $00.00$ &
                   $00.00$ \\                   
%\multirow{10}{*}{}& 
LSUN & 
                   $00.00$ & $92.38$ & $00.00$ & $83.84$ &
                   $95.69$ & $87.74$ & $00.00$ & $00.00$ &
                   $00.00$ \\                   
%\multirow{10}{*}{}& 
STL$10$ & 
                   $00.00$ & $90.50$ & $00.00$ & $80.20$ &
                   $93.35$ & $88.74$ & $94.03$ & $00.00$ &
                   $00.00$ \\
%\multirow{10}{*}{}& 
Places$365$ & 
                   $00.00$ & $91.54$ & $00.00$ & $84.64$ &
                   $95.47$ & $90.34$ & $91.41$ & $00.00$ &
                   $00.00$ \\
%\multirow{10}{*}{}&                   
%Places$365$\textunderscore{b} & 
%                   $00.00$ & $00.00$ & $00.00$ & $00.00$ &
%                   $00.00$ & $00.00$ & $00.00$ & $00.00$ &
%                   $00.00$ \\
                   
%\multirow{10}{*}{}& 
Texture & 
                   $00.00$ & $88.44$ & $00.00$ & $70.94$ &
                   $86.09$ & $90.66$ & $76.87$ & $00.00$ &
                   $00.00$ \\
\hline
Average & 	
                   $00.00$ & $86.25$ & $00.00$ & $81.30$ &
                   $89.01$ & $86.00$ & $85.40$ & $00.00$ &
                   $00.00$ \\
            
\hline
\end{tabularx}
%\end{adjustbox}
%} % end resize box
\end{center}
\end{table*}

==> tab/old_cifar10_Ablation.tex <==
\begin{table*}[t]
%\LARGE
\caption{AUROC scores for OOD Detection with CIFAR$10$ as {$\mathcal{D}^{in}_{train}$} and different $\mathcal{D}_{neg}$. Here, Rotated (Rot.,R) denotes rotated ImageNet images, Debiased is the debiased TinyImageNet dataset, the number after Jigsaw refers to the respective patches, Pixel means that the pixels have been shuffled, In-Dist refers to negative In-Distribution examples and lastly, R.+In-Dist is a combination of the latter one and rotated images.}
\label{tab:contrast_dataset_cif10}
\setlength{\tabcolsep}{2pt}
\begin{center}
%\resizebox{\linewidth}{!}{
%\resizebox{17cm}{2cm}{ % resize table
%\begin{adjustbox}{width=1\textwidth}
%\renewcommand{\arraystretch}{0.3} %change the spacing between rows
\begin{tabularx}{\linewidth}{c*{11}{Y}}
\hline
\multicolumn{1}{c}{$\mathcal{D}^{in}_{train}$: CIFAR$10$} &&\multicolumn{7}{c}{OOD Detection AUROC ($\%$)}
\\
\cline{2-11}
%\multicolumn{1}{c}{$\mathcal{D}_{train}^{in}$} & 
%\multicolumn{1}{c}{$\mathcal{D}_{test}^{out}$} & Vanilla & Normal & Rotated & Debiased & Jigsaw-$16$ & Jigsaw-$4$ & Jig-$4$-Rot & Pixel & In-Dist & R.+In-Dist\\
\multicolumn{1}{c}{$\mathcal{D}_{test}^{out}$} & Vanilla & Standard & R.Aux & R.$360$ & Debiased & Jigsaw-$16$ & Jigsaw-$4$ & R.Jig-$4$ & Pixel & R.In-Dist & R.(Aux+In-Dist)
\hline
% cifar10 as in dist
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\multirow{10}{*}{} 
CIFAR$100$ &
                   $90.29$ & $90.46$ & $92.51$ & $93.77$ &
                   $88.32$ & $89.57$ & $89.29$ & $87.67$ &
                   $93.96$ & $94.25$ \\
%\multirow{10}{*}{}& 
SVHN &  
                   $99.38$ & $99.50$ & $99.62$ & $99.86$ &
                   $99.59$ & $99.13$ & $99.75$& $99.62$ &
                   $99.92$ & $99.92$ \\
%\multirow{10}{*}{}& 
ImageNet$30$ & 
                   $91.41$ & $92.97$ & $97.27$ & $96.04$ &
                   $97.83$ & $82.43$ & $90.43$ & $92.46$ &
                   $93.89$ & $95.34$ \\
%\multirow{10}{*}{}& 
TinyImageNet & 
                   $93.49$ & $88.95$ & $98.00$ & $95.64$ &	
                   $98.80$ & $80.87$ & $91.35$ & $93.89$ &
                   $96.49$ & $97.41$ \\                   
%\multirow{10}{*}{}& 
LSUN & 
                   $91.28$ & $92.71$ & $98.97$ & $99.12$ &
                   $99.52$ & $83.44$ & $92.01$ & $95.63$ &
                   $94.67$ & $97.70$ \\                   
%\multirow{10}{*}{}& 
STL$10$ & 
                   $76.36$ & $84.31$ & $88.34$ & $81.49$ &
                   $92.73$ & $68.78$ & $79.64$ & $83.34$ &
                   $78.16$ & $82.31$ \\
%\multirow{10}{*}{}& 
Places$365$ & 
                   $91.89$ & $94.00$ & $98.36$ & $98.12$ &
                   $99.26$ & $82.90$ & $92.79$ & $94.06$ &
                   $94.44$ & $96.87$ \\
%\multirow{10}{*}{}&                   
%Places$365$\textunderscore{b} & 
%                   $91.86$ & $92.86$ & $98.61$ & $98.12$ &
%                   $99.23$ & $81.56$ & $94.02$ & $94.39$ &
%                   $96.77$ \\
                   
%\multirow{10}{*}{}& 
Texture & 
                   $96.12$ & $96.37$ & $99.72$ & $96.84$ &
                   $99.22$ & $90.14$ & $95.28$ & $94.78$ &
                   $98.46$ & $99.19$ \\
\hline
Average & 	
                   $91.28$ & $92.41$ & $96.65$ & $95.11$ &
                   $96.91$ & $84.66$ & $91.32$ & $92.68$ &
                   $93.75$ & $95.37$ \\ 
            
\hline
\end{tabularx}
%\end{adjustbox}
%} % end resize box
\end{center}
\end{table*}

==> tab/old_sota.tex <==
\begin{table*}[t]
%\small %change the font size
\caption{AUROC scores for OOD detection without label supervision.}
\label{tabl1_sota}
\begin{center}
%\resizebox{13cm}{!}{ % resizing of table
%\begin{adjustbox}{width=1\textwidth, center}
%\renewcommand{\arraystretch}{0.75} %change the spacing between rows
\begin{tabularx}{\textwidth}{c*{8}{Y}}
\hline
&&\multicolumn{6}{c}{OOD Detection AUROC ($\%$)}\\
\cline{3-8}
& & & & & &\multicolumn{2}{c}{\textbf{Ours}}\\
% & & & & & & Ours & Ours\\
%&&\hspace{-2cm}\multicolumn{7}{c}{Ours} \\
{$\mathcal{D}_{train}^{in}$} & {$\mathcal{D}_{test}^{out}$} & Geometric & SSD & CSI & MTL$^*$ &  R. ImgNet & R. ImgNet+R. In-Dist\\ %& Debiased (Ours) \\
\hline
% cifar10 as in dist
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multirow{9}{*}{\rotatebox{90}{CIFAR$10$}} & CIFAR$100$ &
                   $58.21$ & $90.60$ & $89.20$ & $93.24$ & $92.50$ &
                   $\mathbf{94.20}$ \\ % & $93.77$ \\ debiased
%\multirow{8}{*}{}& 
& SVHN & 
                   $77.20$ & $99.60$ & $99.80$ & $\mathbf{99.92}$ & $99.68$  &
                   $\mathbf{99.92}$ \\ % & $99.86$ \\ debiased
%\multirow{8}{*}{}& 
& ImageNet$30$ & 
                   $79.79$ & $90.20$ & $87.92$ & 
                   $-$ & $\mathbf{97.27}$ &
                   $95.34$ \\ %& $96.04$  \\ debiased
%\multirow{8}{*}{}& 
& TinyImageNet & 
                   $76.15$ & $92.30$ & $92.44$& $92.99$ & $\mathbf{98.00}$ &
                   $97.70$ \\ %& $95.64$  \\  debiased         
%\multirow{8}{*}{}& 
& LSUN & 
                   $79.07$ & $96.50$ & $91.60$ & $95.03$ & $\mathbf{98.97}$ &
                   $97.41$ \\ %& \textbf{99.12} \\   debiased                
%\multirow{8}{*}{}& 
& STL$10$ & 
                   $73.55$ & $70.20$ & $64.25$ &
                   $-$ & $\mathbf{88.34}$ &
                   $82.31$ \\ %& $81.49$ \\ debiased
%\multirow{8}{*}{}& 
& Places$365$ & 
                   $77.29$ & $95.20$ & $90.18$ & $93.72$ & $\mathbf{98.74}$ &
                   $96.87$ \\ %& $98.12$ \\ debiased
%\multirow{8}{*}{}& 
& Texture & 
                   $80.26$ & $-$ & $-$ & $-$ & $\mathbf{99.72}$ &
                   $99.19$ \\ % & $96.84$ \\ debiased

\hline
& Average & 
                  $75.19$ & $90.66$ & $87.91$ &
                  $94.98$ & $96.65$ &
                  $95.52$ \\ % & $95.11$ \\ debiased 
                   
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% cifar100 as in dist
\hline \hline

\multirow{7}{*}{\rotatebox{90}{CIFAR$100$}}
& CIFAR$10$& 
                  $48.08$ & $69.60$ & $58.87$ & $\mathbf{79.25}$ & $69.96$ &
                  $68.91$ \\ % & $00.00$ \\ debiased
%\multirow{8}{*}{}& 
& SVHN & 
                  $73.93$ & $94.90$ & $96.44$ & $87.11$ & $96.00$ &
                  $\mathbf{97.51}$ \\ %& $00.00$  \\
%\multirow{8}{*}{}& 
& ImageNet$30$ & 
                  $67.78$ & $75.50$ & $71.82$ &
                  $-$ & $\mathbf{99.35}$ &
                   $86.98$ \\ %& $00.00$ \\                  
%\multirow{8}{*}{}& 
& TinyImagenet & 
                  $60.51$ & $79.50$ & $79.28$ & $80.66$ & $79.89$ &
                  $\mathbf{84.83}$ \\ %& $00.00$ \\
 
%\multirow{8}{*}{}& 
& LSUN & 
                  $70.56$ & $79.50$ & $61.83$ & $74.32$ & $\mathbf{99.74}$ &
                  $83.18$ \\ %& $00.00$ \\                   
%\multirow{8}{*}{}& 
& STL$10$ & 
                  $61.98$ & $72.80$ & $64.26$ & 
                  $-$ & $\mathbf{97.56}$ &
                  $83.12$ \\ %& $00.00$ \\ 
%\multirow{8}{*}{}& 
& Places$365$ & 
                  $67.31$ & $79.60$ & $65.48$ & $77.87$ & $\mathbf{99.26}$ &
                  $82.89$ \\ %& $00.00$ \\

%\multirow{8}{*}{}& 
& Texture & 
                  $68.85$ & $-$ & $-$ &
                  $-$ & $\mathbf{98.75}$ &
                  $88.03$ \\ %& $00.00$ \\ 
\hline
& Average & 
                  $64.88$ & $78.77$ & $71.14$ &
                  $79.84$ & $93.30$ &
                  $84.23$ \\ % & $00.00$ \\  
\hline
\end{tabularx}
%\end{adjustbox}
%} % end resize box
\end{center}
\footnotesize{$^*$Following this method, labels are still required for hyperparameter tuning.}
\end{table*}

%\begin{table}
%\centering
%\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
%\begin{tabular}{@{}lccc@{}}
%\toprule
%Description &  Frobnability \\
%\midrule
%Theirs & Frumpy \\
%Yours & Frobbly \\
%Ours & Makes one's heart Frob\\
%\bottomrule
%\end{tabular}
%} % \resizebox
%\caption{
% 
%\textbf{State of the art} -- Glory to the bold numbers.
% 
%} % \caption
%\label{tab:sota}
%\end{table}

==> tab/old_table2_comparison_AUROC_OOD.tex <==
\begin{table}[t]
\caption{ Comparison results  for OOD detection (AUROC$\%$) with and without overlapping patches. We use (patch size, stride) of $(8,4)$ and $(8,8)$ for with and without overlapping respectively.}
\label{table2_comp_patches_AUROCS}
\begin{center}
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{cccc}
\hline
\multicolumn{3}{r}{Detection AUROC}\\
\cline{3-4}
\multicolumn{1}{c}{$\mathcal{D}_{train}^{in}$} & \multicolumn{1}{c}{$\mathcal{D}_{test}^{out}$} & Without Overlapping &  With Overlapping \\
\hline
\multirow{7}{*}{CIFAR-10} & CIFAR-100 &
                   89.12 & \textbf{90.47} \\
\multirow{7}{*}{}& SVHN & 
                   99.61  & \textbf{99.81} \\
\multirow{7}{*}{}& ImageNet30 & 
                   00.00  & 00.00\\
\multirow{7}{*}{}& TinyImageNet & 
                   94.13  & \textbf{94.61}\\                   
\multirow{7}{*}{}& LSUN & 
                   \textbf{94.97} & 94.40\\                   
\multirow{7}{*}{}& STL10 & 
                   \textbf{74.61}  & 74.07\\ 
\multirow{7}{*}{}& Places365 & 
                   93.50  & \textbf{93.80}\\                    
\hline
\end{tabular}
} %< \resizebox
\end{center}
\end{table}

==> tab/old_table3_comparison_KNN_patches.tex <==
\begin{table}[t]
\caption{ Comparison results  for KNN with and without overlapping patches. We use (patch size, stride) of $(8,4)$ and $(8,8)$ for with and without overlapping respectively. }
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\label{table3_comp_KNN_patches}
\begin{center}
\begin{tabular}{cccc}
\hline
%\multicolumn{3}{r}{Detection AUROC}\\
%\cline{3-4}
 \multicolumn{1}{c}{CIFAR-10} & Without Overlapping &  With Overlapping \\
\hline
10-KNN & 91.45 & \textbf{92.82} \\
20-KNN & 91.76 & \textbf{92.96} \\
\hline
\end{tabular}
\end{center}
} %< \resizebox
\end{table}

==> tab/old_table4_comparison_KNN_AUROC.tex <==
\begin{table}[h!]
\caption{ Comparison results  for KNN and AUROC with and without ImageNet pre-training. We use (patch size, image size) of $(16,224)$ for both senario. Training is done on CIFAR10 dataset.}
\label{table4_KNN_AUROC_imagenet}
\begin{center}
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{cccc}
\hline
%\multicolumn{3}{r}{Detection AUROC}\\
%\cline{3-4}
 \multicolumn{1}{c}{} & Without Pre-Training &  With Pre-Training \\
\hline
10-KNN & 95.65 & \textbf{96.8} \\
\hline
\multicolumn{1}{c}{AUROC} & {} & {}  \\
\hline
 CIFAR100 & 93.57 & \textbf{94.23} \\
 SVHN & \textbf{99.92} & 99.73 \\
 ImageNet30 & \textbf{93.99} & 93.28 \\
 LSUN & \textbf{97.28} & 95.89 \\
 TinyImageNet & 95.58 & \textbf{95.81} \\
 STL10 & 78.45 & \textbf{78.67} \\
 Places365 & \textbf{96.29} & 95.46 \\
\hline
\end{tabular}
} %< \resizebox
\end{center}
\end{table}

==> tab/old_table5_AUROC_without_label_supervision.tex <==
\begin{table*}[ht]
\caption{ AUROC scores for OOD detection without label supervision V2.}
\label{sample-table-v2}
\begin{center}
\begin{adjustbox}{width=1\textwidth}
\begin{tabular}{ccccccccc}
\hline
&&\multicolumn{7}{c}{OOD Detection AUROC ($\%$)}\\
\cline{3-9}
\multicolumn{1}{c}{$\mathcal{D}_{train}^{in}$} & \multicolumn{1}{c}{$\mathcal{D}_{test}^{out}$} & Geometric & SSD & CSI & MTL(Sup) &   In-Dist Neg. (Ours) & Aux-Dist (Ours) & Combined (Ours) \\
\hline
% cifar10 as in dist
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multirow{7}{*}{\rotatebox{90}{CIFAR10}} & 
CIFAR100 &
                   $91.91$ & $90.6$ & $89.2$ & $93.24$ &
                    $94.02$ & $92.50$ &	$\textbf{94.35}$   \\
\multirow{7}{*}{}& 
SVHN & 
                   $97.96$ & $99.6$ & $99.8$ & $99.92$ &
                    $\textbf{99.95}$ &	$99.82$ &	$99.88$ \\
\multirow{7}{*}{}& 
ImageNet30 & 
                   $92.06$ & $90.2$ & $87.92$ & - &
                    $95.05$& $96.82$ &	$\textbf{97.22}$  \\
\multirow{7}{*}{}& 
TinyImageNet & 
                   - & $92.3$ & $92.44$& $92.99$ &
                    $96.30$ &	$96.68$ &	$\textbf{98.80}$  \\                   
\multirow{7}{*}{}& 
LSUN & 
                   $93.57$ & $96.5$ & $91.60$ & $95.03$ &
                    $96.89$	& $98.80$ & $\textbf{99.07}$ \\                   
\multirow{7}{*}{}& 
STL10 & 
                   - & $70.2$ & $64.25$ & - & 
                    $80.61$	& $\textbf{88.52}$ &	$85.60$  \\ 
\multirow{7}{*}{}& 
Places365 & 
                   $92.57$ & $95.2$ & $90.18$ & $93.72$ &
                    $96.23$	& $98.24$ &	$\textbf{98.50}$ \\  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% cifar100 as in dist
\hline \hline

\multirow{7}{*}{\rotatebox{90}{CIFAR100}} & 
CIFAR10 & 
                  $0.74$ & $69.6$ & $58.87$ & 0.00 &
                  0.00 & 00.00 &\textbf{67.36} \\
\multirow{7}{*}{}& 
SVHN & 
                  $0.90$ & $94.9$ & $96.44$ & 0.00 &
                   0.00 & 00.00 &\textbf{97.00} \\
\multirow{7}{*}{}& 
ImageNet30 & 
                  $0.80$ & $75.5$ & $71.82$ & 0.00 &
                  0.00 & 00.00 &\textbf{99.72}\\                  
\multirow{7}{*}{}& 
TinyImagenet & 
                  $0.84$ & $79.5$ & $79.28$ & 0.00 &
                  0.00 & 00.00 &\textbf{99.98}\\
 
\multirow{7}{*}{}& 
LSUN & 
                  $0.81$ & $79.5$ & $61.83$ & 0.00 
                  & 0.00 & 00.00 &\textbf{99.98}\\                   
\multirow{7}{*}{}& 
STL10 & 
                  $0.84$ & $72.8$ & $64.26$ & 0.00 &
                  0.00 & 00.00 &\textbf{99.92}\\ 
\multirow{7}{*}{}& 
Places365 & 
                  $0.81$ & $79.6$ & $65.48$ & 0.00 &
                  0.00 & 00.00 &  \textbf{99.96} \\  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%     
% ImageNet30 in dist
 \hline \hline                 
\multirow{7}{*}{\rotatebox{90}{ImageNet30}} & 
CIFAR10 & 
                  $0.95$ & 0.00 & 0.00 & 0.00 &
                  0.00 & 00.00 &\textbf{89.96} \\
\multirow{7}{*}{}& 
CIFAR100 & 
                  $0.96$ & 0.00 & 0.00 & 0.00 &
                  0.00 & 00.00 &\textbf{92.51} \\                  
\multirow{7}{*}{}& 
SVHN & 
                  $0.97$ & 0.00 & 0.00 & 0.00 & 
                  0.00 & 00.00 &\textbf{99.11} \\
\multirow{7}{*}{}& 
TinyImagenet & 
                  $0.91$ & 0.00 & 0.00 & 0.00 &
                  0.00 & 00.00 &\textbf{89.25}\\
\multirow{7}{*}{}& 
LSUN & 
                  $0.86$ & 0.00 & 0.00 & 0.00 &
                  0.00 & 00.00 &\textbf{67.72}\\                   
\multirow{7}{*}{}& 
STL10 & 
                  $0.88$ & 0.00 & 0.00 & 0.00 &
                  0.00 & 00.00 &\textbf{76.22}\\ 
\multirow{7}{*}{}& 
Places365 & 
                  $0.88$ & 0.00 & 0.00 & 0.00 &
                  0.00 & 00.00 &\textbf{71.19}\\                    
                
\hline
\end{tabular}
\end{adjustbox}
\end{center}
\end{table*}

==> tab/old_table6_v2_temp_imagenet.tex <==
\begin{table}[t]
\caption{v2, $temp_{initial}^t$ = $0.055$}
\label{table6_v2_temp}
\begin{center}
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{cccccc}
\hline
\multicolumn{5}{r}{OOD Detection AUROC ($\%$)}\\
\cline{3-6}
\multicolumn{1}{c}{$\mathcal{D}_{train}^{in}$} & \multicolumn{1}{c}{$\mathcal{D}_{test}^{out}$} & CSI &  In-Dist Neg & Aux-Dist & Combined\\
\hline
\multirow{7}{*}{ImageNet30} & CIFAR-100 &
                   &89.13 & \textbf{96.40} & 93.96\\
\multirow{7}{*}{} & CIFAR-10 &
                   &84.08 & \textbf{95.19} &92.97 \\                   
\multirow{7}{*}{}& SVHN & 
                   &99.50  & \textbf{99.99} & 99.97\\

\multirow{7}{*}{}& TinyImageNet & 
                   &65.85  & \textbf{69.13} & 65.53\\                   
\multirow{7}{*}{}& LSUN & 
                   &46.72 & 54.05 & \textbf{63.14}\\                   
\multirow{7}{*}{}& STL10 & 
                   &60.14  & \textbf{69.14} & 66.75\\ 
\multirow{7}{*}{}& Places365 & \textbf{78.3}
                   &50.29  & 57.11 & 63.78\\   
\multirow{7}{*}{}& Texture & 
                  & \textbf{65.98}  & 53.41 & 55.41\\                   
\hline
\end{tabular}
} %< \resizebox
\end{center}
\end{table}

==> tab/old_table7_D_in_train_Imagenet.tex <==
\begin{table*}[ht]
\caption{{$\mathcal{D}_{train}^{in}$}:ImageNet30, v3}
\label{table7_Din_imagenet}
\begin{center}
\resizebox{13cm}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{ccccccc}
\hline
&&{$temp_{initial}^t$ = $0.055$}&&&{$temp_{initial}^t$ = $0.04$}\\
\cline{2-7}
{$\mathcal{D}_{test}^{out}$} & In-Dist Neg & Aux-Dist & Combined & In-Dist Neg & Aux-Dist & Combined\\
\hline
CIFAR-100 &
                   89.27&\textbf{96.20}& 62.88 &90.39&95.39&93.52 \\
 CIFAR-10 &
                  89.57&\textbf{95.93}&70.36 &87.55&94.19& 90.45\\                   
SVHN & 
                   93.63&99.22& 68.13 &98.81&\textbf{99.40}&99.33\\
TinyImageNet & 
                   86.44&\textbf{94.27}&66.15&86.90&92.55&90.23\\                   
LSUN & 
                   60.74&69.50&\textbf{72.28} &67.04 &71.72&66.22\\                   
STL10 & 
                   69.17&78.57&64.41 &73.26 &\textbf{79.13}&75.24\\ 
Places365 & 
                   64.92&72.94&67.97 &70.84&\textbf{75.32}& 70.45\\
Texture & 
                   84.24 & 92.98 & 57.48 &90.32&90.94& \textbf{93.33}\\
\hline
\end{tabular}
} %< \resizebox
\end{center}
\end{table*}


==> tab/old_table8_v2_temp_cifar100.tex <==
\begin{table}[t]
\caption{v2, $temp_{initial}^t$ = $0.055$}
\label{table8_v2}
\begin{center}
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{cccc}
\hline
\multicolumn{4}{r}{OOD Detection AUROC ($\%$)}\\
\cline{3-4}
\multicolumn{1}{c}{$\mathcal{D}_{train}^{in}$} & \multicolumn{1}{c}{$\mathcal{D}_{test}^{out}$} & Aux-Dist & Combined\\
\hline
\multirow{7}{*}{CIFAR-100} & CIFAR-10 
&70.24&68.10\\
\multirow{7}{*}{}& SVHN 
&90.47&96.04\\                   
\multirow{7}{*}{} & ImageNet30  
&99.21&79.74\\                   
\multirow{7}{*}{}& TinyImageNet  
&82.57&77.67\\                   
\multirow{7}{*}{}& LSUN  
&99.58&77.44\\                   
\multirow{7}{*}{}& STL10  
&94.66&77.50\\ 
\multirow{7}{*}{}& Places365  
&99.44&77.89\\   
\multirow{7}{*}{}& Texture  
&97.71&75.75\\                   
\hline
\end{tabular}
} %< \resizebox
\end{center}
\end{table}



==> tab/old_table9_D_in_train_Cifar100.tex <==
\begin{table}[t]
\caption{{$\mathcal{D}_{train}^{in}$}:CIFAR-100, v3, $temp_{initial}^t$ = $0.05$}
\label{table9_Din_cifar100}
\begin{center}
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{ccccc}
\hline
\multicolumn{4}{r}{OOD Detection AUROC ($\%$)}\\
\cline{2-5}
{$\mathcal{D}_{test}^{out}$} & In-Dist Neg & Aux-Dist & Combined & Combined\\
\hline
CIFAR-10 &67.07&69.96&67.06&68.91\\                   
SVHN &97.95&0.96&96.74&97.51\\ 
ImageNet30 &79.46&99.35&82.21&86.98\\ 
TinyImageNet &79.85 &79.89&76.90&84.83\\ 
LSUN & 74.31&99.74&82.15&83.18\\ 
STL10 &72.24&97.56&79.70&83.12\\ 
Places365 &75.26&99.26&80.67&82.89\\ 
Texture &78.11 &98.75&76.80&88.03\\ 
\hline
\end{tabular}
} %< \resizebox
\end{center}
\end{table}
